End-to-end learned Lossy Dynamic Point Cloud Attribute Compression

Recent advancements in point cloud compression have primarily emphasized geometry compression while comparatively fewer efforts have been dedicated to attribute compression. This study introduces an end-to-end learned dynamic lossy attribute coding approach, utilizing an efficient high-dimensional convolution to capture extensive inter-point dependencies. This enables the efficient projection of attribute features into latent variables. Subsequently, we employ a context model that leverage previous latent space in conjunction with an auto-regressive context model for encoding the latent tensor into a bitstream. Evaluation of our method on widely utilized point cloud datasets from the MPEG and Microsoft demonstrates its superior performance compared to the core attribute compression module Region-Adaptive Hierarchical Transform method from MPEG Geometry Point Cloud Compression with 38.1% Bjontegaard Delta-rate saving in average while ensuring a low-complexity encoding/decoding.

==> basic-block-diagram.tex <==

	
	\begin{adjustbox}{width=0.5\textwidth}
%		\tikzstyle{font} = {definition}
		


	\tikzset{every picture/.style={line width=0.75pt}} %set default line width to 0.75pt        

\begin{tikzpicture}[x=0.75pt,y=0.75pt,yscale=-1,xscale=1]
	%uncomment if require: \path (0,466); %set diagram left start at 0, and has height of 466
	
		%Straight Lines  l1 start
	\draw    (125,180.88) -- (157.63,180.88) ;
	\draw [shift={(160.63,180.88)}, rotate = 180] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (8.93,-4.29) -- (0,0) -- (8.93,4.29) -- cycle    ;
	
	
	%Straight Lines  l1 short
	\draw    (257.86,180.88) -- (303.75,180.88) ;
	\draw [shift={(306.75,180.88)}, rotate = 180] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (8.93,-4.29) -- (0,0) -- (8.93,4.29) -- cycle    ;
	
		
	
	%Straight Lines l1 long
	\draw    (341,180) -- (623.07,181.1) ;
	\draw [shift={(626.07,181.11)}, rotate = 180.22] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (8.93,-4.29) -- (0,0) -- (8.93,4.29) -- cycle    ;
	
	
	
	
	%Straight Lines  l1 last
	\draw  [dash pattern={on 4.5pt off 4.5pt}]  (730.81,180.88) -- (773,180.88) ;
	\draw [shift={(776,180.88)}, rotate = 180] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (8.93,-4.29) -- (0,0) -- (8.93,4.29) -- cycle    ;
	
	
	
	%Straight Lines  l2 short
	\draw    (318.48,353.94) -- (364.37,353.94) ;
	\draw [shift={(367.37,353.94)}, rotate = 180] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (8.93,-4.29) -- (0,0) -- (8.93,4.29) -- cycle    ;
	%Straight Lines  l2 long
	\draw    (407,353.94) -- (562.89,354.96) ;
	\draw [shift={(565.89,354.98)}, rotate = 180.38] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (8.93,-4.29) -- (0,0) -- (8.93,4.29) -- cycle    ;






	%Straight Lines l1 c l2 
	\draw    (279.37,180.88) -- (279.37,330.06) ;
	\draw [shift={(279.37,333.06)}, rotate = 270] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (8.93,-4.29) -- (0,0) -- (8.93,4.29) -- cycle    ;
	%Straight Lines l3
	\draw    (376.17,527) -- (413.06,527) ;
	\draw [shift={(416.06,527)}, rotate = 180] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (8.93,-4.29) -- (0,0) -- (8.93,4.29) -- cycle    ;
	%Straight Lines  l3
	\draw    (433.3,527) -- (508.63,527) ;
	\draw [shift={(511.63,527)}, rotate = 180] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (8.93,-4.29) -- (0,0) -- (8.93,4.29) -- cycle    ;

	%Straight Lines  l2 c l3
	\draw    (337.06,353.94) -- (337.06,503.13) ;
	\draw [shift={(337.06,506.13)}, rotate = 270] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (8.93,-4.29) -- (0,0) -- (8.93,4.29) -- cycle    ;
	
	%Straight Lines  up l3 to l2
	\draw    (613.47,527) -- (633.03,527) -- (633.03,377.82) ;
	\draw [shift={(633.03,374.82)}, rotate = 90] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (8.93,-4.29) -- (0,0) -- (8.93,4.29) -- cycle    ;



	%Straight Lines  up l2 to l1
	\draw    (666.14,353.94) -- (685.7,353.94) -- (685.7,204.75) ;
	\draw [shift={(685.7,201.75)}, rotate = 90] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (8.93,-4.29) -- (0,0) -- (8.93,4.29) -- cycle    ;

	%Straight Lines  l2 last
	\draw  [dash pattern={on 4.5pt off 4.5pt}]  (685.7,353.94) -- (767,353.94) ;
	\draw [shift={(770,353.94)}, rotate = 180] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (8.93,-4.29) -- (0,0) -- (8.93,4.29) -- cycle    ;
	%Straight Lines l3 last
	\draw  [dash pattern={on 4.5pt off 4.5pt}]  (633.03,527) -- (773,527) ;
	\draw [shift={(776,527)}, rotate = 180] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (8.93,-4.29) -- (0,0) -- (8.93,4.29) -- cycle    ;

	
	

		%Shape: Rectangle  encoder1
	\draw  [color={rgb, 255:red, 22; green, 58; blue, 68 }  ,draw opacity=1 ][fill={rgb, 255:red, 219; green, 238; blue, 243 }  ,fill opacity=1 ] (161,160) -- (261,160) -- (261,201.75) -- (161,201.75) -- cycle ;
	%Shape: Rectangle  decoder1
	\draw  [color={rgb, 255:red, 86; green, 40; blue, 4 }  ,draw opacity=1 ][fill={rgb, 255:red, 253; green, 235; blue, 221 }  ,fill opacity=1 ] (627.59,160) -- (727.59,160) -- (727.59,201.75) -- (627.59,201.75) -- cycle ;
		%Rounded Rectq1
	\draw  [color={rgb, 255:red, 51; green, 63; blue, 27 }  ,draw opacity=1 ][fill={rgb, 255:red, 235; green, 241; blue, 223 }  ,fill opacity=1 ] (306.75,168.35) .. controls (306.75,163.74) and (310.48,160) .. (315.1,160) -- (340.19,160) .. controls (344.81,160) and (348.55,163.74) .. (348.55,168.35) -- (348.55,193.4) .. controls (348.55,198.01) and (344.81,201.75) .. (340.19,201.75) -- (315.1,201.75) .. controls (310.48,201.75) and (306.75,198.01) .. (306.75,193.4) -- cycle ;
	% Text Node
	\draw (209,180) node [anchor=center][inner sep=0.75pt]  [font=\small,xscale=2.25,yscale=2.25] [align=left] {Enc. I};
	% Text Node
	\draw (327,180) node [anchor=center][inner sep=0.75pt]  [font=\small,xscale=2.25,yscale=2.25] [align=left] {Q};
	% Text Node
	\draw (676,180) node [anchor=center][inner sep=0.75pt]  [font=\small,xscale=2.25,yscale=2.25] [align=left] {Dec. I};
	
	
	
			%Shape: Rectangle  encoder2
	\draw  [color={rgb, 255:red, 22; green, 58; blue, 68 }  ,draw opacity=1 ][fill={rgb, 255:red, 219; green, 238; blue, 243 }  ,fill opacity=1 ] (217.25,333.06) -- (317.25,333.06) -- (317.25,374.82) -- (217.25,374.82) -- cycle ;
		%Shape: Rectangle  %decoder 2
	\draw  [color={rgb, 255:red, 86; green, 40; blue, 4 }  ,draw opacity=1 ][fill={rgb, 255:red, 253; green, 235; blue, 221 }  ,fill opacity=1 ] (565.92,333.06) -- (665.92,333.06) -- (665.92,374.82) -- (565.92,374.82) -- cycle ;
		%Rounded Rect q2
	\draw  [color={rgb, 255:red, 51; green, 63; blue, 27 }  ,draw opacity=1 ][fill={rgb, 255:red, 235; green, 241; blue, 223 }  ,fill opacity=1 ] (367.09,341.61) .. controls (367.09,337) and (370.83,333.26) .. (375.44,333.26) -- (400.54,333.26) .. controls (405.16,333.26) and (408.89,337) .. (408.89,341.61) -- (408.89,366.66) .. controls (408.89,371.28) and (405.16,375.01) .. (400.54,375.01) -- (375.44,375.01) .. controls (370.83,375.01) and (367.09,371.28) .. (367.09,366.66) -- cycle ;
		% Text Node
	\draw (266,354) node [anchor=center][inner sep=0.75pt]  [font=\small,xscale=2.25,yscale=2.25] [align=left] {Enc. II};
		% Text Node
	\draw (388,354) node [anchor=center][inner sep=0.75pt]  [font=\small,xscale=2.25,yscale=2.25] [align=left] {Q};
	% Text Node
	\draw (615,354) node [anchor=center][inner sep=0.75pt]  [font=\small,xscale=2.25,yscale=2.25] [align=left] {Dec. II};
	
	
	
	
	
	
	
		%Shape: Rectangle %encoder 3
	\draw  [color={rgb, 255:red, 22; green, 58; blue, 68 }  ,draw opacity=1 ][fill={rgb, 255:red, 219; green, 238; blue, 243 }  ,fill opacity=1 ] (275.94,506.13) -- (375.94,506.13) -- (375.94,547.88) -- (275.94,547.88) -- cycle ;
	%Shape: Rectangle decoder 3
	\draw  [color={rgb, 255:red, 86; green, 40; blue, 4 }  ,draw opacity=1 ][fill={rgb, 255:red, 253; green, 235; blue, 221 }  ,fill opacity=1 ] (512.25,506.13) -- (612.25,506.13) -- (612.25,547.88) -- (512.25,547.88) -- cycle ;
	
		%Rounded Rect q3
	\draw  [color={rgb, 255:red, 51; green, 63; blue, 27 }  ,draw opacity=1 ][fill={rgb, 255:red, 235; green, 241; blue, 223 }  ,fill opacity=1 ] (416.08,514.48) .. controls (416.08,509.87) and (419.82,506.13) .. (424.43,506.13) -- (449.53,506.13) .. controls (454.14,506.13) and (457.88,509.87) .. (457.88,514.48) -- (457.88,539.53) .. controls (457.88,544.14) and (454.14,547.88) .. (449.53,547.88) -- (424.43,547.88) .. controls (419.82,547.88) and (416.08,544.14) .. (416.08,539.53) -- cycle ;
	
		% Text Node
	\draw (324,527) node [anchor=center][inner sep=0.75pt]  [font=\small,xscale=2.25,yscale=2.25] [align=left] {Enc. III};
		% Text Node
	\draw (436,527) node [anchor=center][inner sep=0.75pt]  [font=\small,xscale=2.25,yscale=2.25] [align=left] {Q};
	% Text Node
	\draw (561.5,527) node [anchor=center][inner sep=0.75pt]  [font=\small,xscale=2.25,yscale=2.25] [align=left] {Dec. III};
	










	% Text Node
\draw (750,214) node [anchor=west][inner sep=0.75pt]  [font=\small,xscale=2.5,yscale=2.5]  {$z^{1}$};	
% Text Node
\draw (675,387) node [anchor=west][inner sep=0.75pt]  [font=\small,xscale=2.5,yscale=2.5]  {$z^{2}$};
% Text Node
\draw (621,560) node [anchor=west][inner sep=0.75pt]  [font=\small,xscale=2.5,yscale=2.5]  {$z^{3}$};



	% Text Node
\draw (470,209) node [anchor=west][inner sep=0.75pt]  [font=\small,xscale=2.5,yscale=2.5]  {$L^{1}$};	
\draw (470,383) node [anchor=west][inner sep=0.75pt]  [font=\small,xscale=2.5,yscale=2.5]  {$L^{2}$};	
% Text Node
\draw (470,556) node [anchor=west][inner sep=0.75pt]  [font=\small,xscale=2.5,yscale=2.5]  {$L^{3}$};	




% Text Node
\draw (804,180) node [anchor=west][inner sep=0.75pt]  [font=\small,xscale=2.5,yscale=2.5]  {$p( F\ |\ z^{1})$};

% Text Node
\draw (804,354) node [anchor=west][inner sep=0.75pt]  [font=\small,xscale=2.5,yscale=2.5]  {$p( L^{1} \ |\ z^{2})$};	
	% Text Node
\draw (804,527) node [anchor=west][inner sep=0.75pt]  [font=\small,xscale=2.5,yscale=2.5]  {$p( L^{2} \ |\ z^{3})$};


% Text Node
\draw (90,180) node [anchor=west][inner sep=0.75pt]  [font=\small,xscale=2.5,yscale=2.5]  {$F$};
	
	
	
	
\end{tikzpicture}

	
\label{systemooverview}
		
\end{adjustbox}


==> maskAlgo.tex <==
\begin{algorithm2e}[h]
\SetAlgoLined
\SetKwInOut{Input}{Input}
 \small
%\SetKwInOut{Output}{Output}
\KwIn{$mask\_type$} 
%\KwOut{partitioning flags: $fl$, output bitstream: $bits$}
$kernel\_size \leftarrow k_D*k_H*k_W$\\
$mask \leftarrow$ $ ones\_like(kernel)$\\
$mask\left[kernel\_size//2+ mask\_type==B,:,: \right]=0$\\
$kernel=kernel*mask$
       
\caption{Mask construction and application}
\label{algo:maskalg}
\end{algorithm2e}
%\setlength{\textfloatsep}{0pt}
% $kernel\_size=kernel.size()$\\

==> proposemethod.tex <==

\subsection{Auto-Encoder and Rate-Distortion Optimization}
%\input{basic-block-diagram}
\begin{figure}
\centering
\captionsetup{justification=justified}
% \captionsetup{singlelinecheck = false, format= hang, justification=raggedright, font=small, labelsep=space}
\includegraphics[width=.95\linewidth]{figures_pcc/mscale.png}
\vspace{0.1cm}
\caption{System overview of the proposed method MNeT. At each scale, we have three components: Encoder (blue), a Quantizer (green), and a Decoder (light grown). All latent representation (L) and RGB feature (F) are encoded to bitstream using the predicted probability distribution from the decoders, except the last layer where we encode $L^3$ using a uniform distribution.   }
\label{fig:3Dcontext}
\end{figure}

\par The details of our novel method will be presented in this section. We represent the attributes of each point cloud frame using a spare tensors \{C, F\} given that the coordinates of occupied voxels  $C=\{x_i,y_i,z_i\}_i$ are already known. We aim to encode each frame's feature set $F$ that is composed of red, green, and blue (RGB) colors, or other attributes such as YUV colors, normals, velocities, etc. Our approach to lossy encoding is to learn a latent variable model in which the latent variables capture the important feature to be transmitted and reconstructed at the decoder. 

\begin{equation} \label{eq:factorization}
\begin{split}
   p(F, L^{1,..,N})=p(F|L^{1,..,N}) \cdot \prod_{n=1}^{N} &p(L^n|L^{n+1}, .., L^N) 
\end{split}
\end{equation}

\begin{figure*}
\centering
\captionsetup{justification=justified}
% \captionsetup{singlelinecheck = false, format= hang, justification=raggedright, font=small, labelsep=space}
\includegraphics[width=.83\linewidth]{figures_pcc/networkarchitecture_mnet.png}
\vspace{0.1cm}
\caption{MNeT network architecture for a single scale including an \textbf{Encoder}, a Quantizer \textbf{Q} and a \textbf{Decoder}. SP-ConV and ST-Conv denote the sparse convolution and sparse transpose convolution with convolution kernel and stride denoted using kKsS (kernel K, stride S). We use the same number of output filters (filter=64) for all convolution layers, except the one before quantization (filter=5) and the last convolution layer at the decoder (filter $\in$ [120, 150, 150]).}
\label{fig:network}
\end{figure*}

Each term on the right-hand side is the joint probability of latent representation $L^n$ or the RGB color $F$ given all lower scales. However, instead of directly modeling the upper latent representation from the lower scales $p( L^n|  L^{n+1},..., L^N)$, the decoders are modeled such that
\begin{equation} \label{eq:factorization}
\begin{split}
   p( L^n|  L^{n+1},..., L^N)
   &=p(L^n|z^{n+1})
\end{split}
\end{equation}
with $z^{n+1}$ is considered as a sumerization of $L^{n+1,..,N}$. Auto-regressive modeling has been shown as the state-of-the-art method for estimating data likelihood \cite{salimans2017pixelcnn++,nguyen2022learning} by learning the dependencies between sub-points/pixels. However, in this work, we do not factorize the probability $p(F)$ over sub-points, which can lead to a significant number of network evaluations. Instead, we assume that all sub-points are statistically independent and jointly model all the sub-points together while keeping the relation between RGB channels within each sub-point. Specifically, for each sub-point feature $f_i$ of F, we factorize the joint distribution as: 
\begin{equation} \label{eq:factorization}
\begin{split}
   p(f_i|z^1)&=p(f_{i}^{RGB}|z^1)\\
   &=p(f_{i}^{R}|z^1) \cdot p(f_{i}^{G}|f_{i}^{R},z^1) \cdot p(f_{i}^{B}|f_{i}^{R},f_{i}^{G},z^1)
\end{split}
\end{equation}
Each probability distribution on the right hand side is modeled via discretized logistic mixture model proposed in \cite{salimans2017pixelcnn++}. Specifically, we first model the distribution of the red channel using information from the lower latent as a mixture of $K$ logistic distributions. Next, we predict the green channel using the same principle, but we allow the means of mixture components to linearly depend on the value of the red channel. Similarly, in the blue channel, the mean of the mixture coefficients depends on the values of the red and green channels. On the lower scales, we also use a logistic mixture to model the latent distributions, but we do not enforce any dependencies between channels. 

\par In order to learn good predictions $\hat{p}(F, L^1,..., L^N)$  of the joint color attribute and latent distribution $p(F, L^1,..., L^N)$ and thus minimize the encoding bitrate, we train the auto-encoders by minimizing the total cross-entropy losses on all latent representations: 
\begin{equation} \label{eq:lossfunction}
\begin{split}
   Loss &= H(\hat{p},p)=H(\hat{p}_{F|z^1},p_{F|z^1}) + H(\hat{p}_{L^1|z^2},p_{L^1|z^2})  \\
   &+H(\hat{p}_{L^2|z^3},p_{L^2|z^3}) +H(\hat{p}_{L^3},p_{L^3}) 
\end{split}
\end{equation}



\subsection{Network Architecture}
\par The architecture of an auto-encoder for a single scale is presented in Figure \ref{fig:network}. At the encoder side, we first apply a convolution followed by a Max-Pooling layer. We find that aggregating a convolution layer with a Max-Pooling provides faster training and better performance compared with a single convolution layer with stride=2. Next, we deploy 8 residual blocks followed by two convolution layers in two branches: one going to the quantization (filter=5) and one going to the lower scale (filter=64). The MNeT residual blocks are inspired by the 2D residual block from EDSR \cite{lim2017enhanced} as our multi-scale prediction is similar to super-resolution tasks. We adopt the scalar quantization from \cite{mentzer2019practical} which allows gradient back propagation during training. We set the number of bins to 26 in all the quantizers. At the decoder side, which takes inputs from the quantization and the lower scale, we first apply a convolution layer followed by 8 residual blocks, an upsampler, and convolutions. The decoders output the logistic mixture parameters for probability construction and the forwarding feature for the upper scale.  In this work, we use 10 mixture of logistics on every scale, thus the number of decoders' output channels are 120, 150, 150 from the top scale to the bottom scale, respectively.
\input{compare-methods-table}
\subsection{Encoder and Decoder}

==> resultTable.tex <==

\begin{table}[t]
\caption{Comparions of our method against G-PCC v14 and VoxelDNN}
\resizebox{0.99\linewidth}{!}{ \begin{tabular}{|P{0.1cm}|l|P{1.2cm}||R{0.7cm}|R{1.4cm}|R{0.7cm}|R{1.4cm}|}
\cline{3-7}
% \multicolumn{2}{|c||}{\begin{bf} Test PC \end{bf}}
\multicolumn{2}{c|}{}
& \begin{bf} G-PCC \end{bf}
& \multicolumn{2}{c|}{\begin{bf}VoxelDNN\end{bf}}
& \multicolumn{2}{c|}{\begin{bf}SparseVoxelDNN\end{bf}}
\\
\cline{2-7}
\multicolumn{1}{c|}{}&Point Cloud & bpov&bpov&Gain over G-PCC &bpov&Gain over G-PCC\\
\hline

\multirow{3}{*}{\rotatebox[origin=c]{90}{MVUB}}&Phil& 1.15 &0.82 &-28\%& 0.40 &-66\%  \\ 
\cline{2-7}
&Ricardo&1.07 &0.75 &-29\%& 0.35&-67\% \\
\cline{2-7}
&\textbf{Average}  &\textbf{1.11}  &\textbf{0.79} &\textbf{-28.5\%} & \textbf{0.37}&\textbf{-66.4\%}  \\
\cline{2-7}
\hline



\multirow{5}{*}{\rotatebox[origin=c]{90}{8i}}&Redandblack &1.09  &0.70 &-36\%& 0.30&-64\% \\
\cline{2-7}
&Loot &0.95&0.61 &-36\% &0.33 & -65\%\\
\cline{2-7}
&Thaidancer&1.00 &0.66 &-34\%&0.32 &-68\% \\
\cline{2-7}
&Boxer&0.95  &0.59 &-38\%& 0.30&-68\% \\
\cline{2-7}
&\textbf{Average} &\textbf{1.00} &\textbf{0.64}& \textbf{-36.0\%}&\textbf{0.34} &\textbf{-66.5\%} \\
\hline



\multirow{4}{*}{\rotatebox[origin=c]{90}{CAT1}}&Frog &1.92   &1.70 &-10\%& 1.23&-36\%  \\
\cline{2-7}
&Arco Valentino &4.85 &4.99 &+3\%& 3.03&-38\% \\
\cline{2-7}
&Shiva&3.67 & 3.50 &-4\%&2.66&-28\% \\
\cline{2-7}
&\textbf{Average} &\textbf{3.48} &\textbf{3.40} &\textbf{-3.8\%}&\textbf{2.31} &\textbf{-33.6\%}\\
\hline



\multirow{3}{*}{\rotatebox[origin=c]{90}{USP}}&BumbaMeuBoi&5.41   &5.07 &-6\%& 2.52&-53\%  \\
\cline{2-7}
&RomanOiLight& 1.86  &1.62 &-13\%& 1.52&-19\% \\
\cline{2-7}
&\textbf{Average}  &\textbf{3.64}  &\textbf{3.35} &\textbf{-9.6\%}&\textbf{2.02}&\textbf{-35.8\%}  \\
\cline{2-7}

\hline
\hline
\end{tabular}}
\label{table:resulttable}
%\noalign{
\vskip 3mm  
\end{table}


==> training_set.tex <==
\begin{table}[t]
\caption{Number of blocks in the training sets of each model}
\centering
\resizebox{0.9\linewidth}{!}{
\begin{tabular}{lR{0.8cm}R{0.8cm}R{0.8cm}R{1.2cm}R{1cm}}
\hline
\begin{bf}  \end{bf}
&\begin{bf}MVUB\end{bf}
& \begin{bf}8i\end{bf} 
&\begin{bf}CAT1\end{bf}
& \begin{bf}Owlii\end{bf} 
& \begin{bf}Total\end{bf} \\
\hline
Block 64 & 317763 &235369 & 2499 & 358834 & 914465\\
\hline
\vspace{0.1mm}
\end{tabular}}
\label{table:noblocks}
\end{table}
